Bi-Level Optimal Control Framework For Missed-Thrust-Design With First-Order Bounds On Maximum Missed-Thrust-Duration

In this paper, we present a bi-level optimal control framework for designing low-thrust spacecraft trajectories with robustness against missed-thrust-events. The upper-level (UL) problem generates a nominal trajectory assuming full control authority, while each lower-level (LL) problem computes the optimal recovery maneuver following a missed-thrust-event along the nominal solution. Under suitable regularity conditions ensuring uniqueness and smoothness of the LL response, the hierarchy admits a single-level reformulation by embedding the LL first-order optimality conditions within the UL constraints. We further establish a robustness certificate, which provides an upper bound on the maximum admissible missed-thrust-duration for which the structural assumptions remain valid for the LL problem. The bound depends explicitly on precomputable dynamical quantities along the nominal solution, enabling rapid evaluation over large ensembles without iterative solves. Numerical experiments show that while the certificate identifies when modeling assumptions are valid, it does not fully characterize recoverability after missed-thrust-events. A finite-horizon controllability-energy analysis is therefore used to interpret recovery beyond the theoretical bounds. Collectively, these results provide a deterministic, certifiable approach for incorporating robustness directly into trajectory design, replacing post-hoc margin allocation techniques with formal guarantees.

==> review/reviewers/meta.tex <==
% Response to Editor
\editor
\begin{generalcomment}
    The reviewer(s) have suggested some revisions to your manuscript. Therefore, I invite you to respond to the reviewer(s)' comments and revise your manuscript.
\end{generalcomment}
\begin{revmeta}[]
We are grateful for the opportunity to address the reviewers' comments on the manuscript, \emph{A Bi-Level Optimal Control Framework for Low-Thrust Trajectory Design under Missed-Thrust-Events} (Manuscript ID: 202X-XY-GZZZZZZ), to be considered for publication in the \emph{Journal of Guidance, Control, and Dynamics}.
We are thankful to the reviewers for their comments and questions which have led to significant improvements in the overall quality of the manuscript.
We believe that these changes have substantially improved the manuscript and we hope you will find that it merits publication.
Below, we provide detailed responses to each comment from the reviewers.
Any changes to the manuscript, in response to the reviewers' comments, have been highlighted in \hlone{yellow} in the updated manuscript, and are reproduced in this document following each reviewer comment.
Any additional changes made by the author are highlighted in \hltwo{cyan} in the updated manuscript, but have not been reproduced in this document. 
\end{revmeta}

==> review/reviewers/r1.tex <==
% Reviewer 1
\reviewer
\begin{revcomment}
    \begin{quote}
        ``asd''
    \end{quote}
    asd
\end{revcomment}
\begin{revresponse}
    asd
    \begin{changes}[\S X Page YY, Line ZZZ - Page YY, Line ZZZ]
        asd
    \end{changes}
\end{revresponse}


==> review/reviewers/r2.tex <==
% Reviewer 1
\reviewer
\begin{revcomment}
    \begin{quote}
        ``asd''
    \end{quote}
    asd
\end{revcomment}
\begin{revresponse}
    asd
    \begin{changes}[\S X Page YY, Line ZZZ - Page YY, Line ZZZ]
        asd
    \end{changes}
\end{revresponse}


==> sections/funding_sources.tex <==
\section*{Funding Sources}
\astodos{Need to write this section}
